A Novel Approach for Intrinsic Dimension Estimation

The real-life data have a complex and non-linear structure due to their nature. These non-linearities and the large number of features can usually cause problems such as the empty-space phenomenon and the well-known curse of dimensionality. Finding the nearly optimal representation of the dataset in a lower-dimensional space (i.e. dimensionality reduction) offers an applicable mechanism for improving the success of machine learning tasks. However, estimating the required data dimension for the nearly optimal representation (intrinsic dimension) can be very costly, particularly if one deals with big data. We propose a highly efficient and robust intrinsic dimension estimation approach that only relies on matrix-vector products for dimensionality reduction methods. An experimental study is also conducted to compare the performance of proposed method with state of the art approaches.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}



==> tablolar.tex <==
\begin{table}[]
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Dataset & ID & PM & $PM_{Spec}$ & $PM_{Kmeans}$ &PFO & PFN & PMG & PRT & PPR & PKS & PBS & CID & FSH & KNN & MADA & $Mind_{ML}$ & MLE & MOM & TLE & TNN & DANCo & ESS \\ 
\hline
$\mathcal{M}_1$ & \textbf{10.00} & 9.00 & 8.00 & 8.00 & 11.00 & 7.00 & 1.00 & 1.00 & 10.94 & 5.00 & 1.00 & 8.91 & 11.02 & 11.00 & 9.62 & 9.10 & 9.53 & 8.60 & 10.10 & 9.28 & 11.00 & 10.18 \\ 
\hline
$\mathcal{M}_2$ & \textbf{3.00} & 2.00 & 2.00 & 3.50 & \textbf{3.00} & 2.00 & \textbf{3.00} & 1.00 & 2.27 & 2.00 & \textbf{3.00} & 2.87 & 2.92 & 4.00 & 3.07 & 2.90 & 3.03 & 2.79 & 3.13 & 2.92 & 2.96 & 2.90 \\ 
\hline
$\mathcal{M}_3$ & \textbf{4.00} & 2.00 & 3.00 & 5.00 & 5.00 & 2.00 & 2.00 & 1.00 & 2.75 & 2.00 & 3.00 & 3.58 & 3.34 & 1.00 & 4.14 & 3.77 & 4.03 & 3.77 & 4.21 & 3.79 & 4.67 & 4.02 \\ 
\hline
$\mathcal{M}_4$ & \textbf{4.00} & 8.00 & \textbf{4.00} & 5.50 & 8.00 & 5.00 & 1.00 & 1.00 & 7.96 & \textbf{4.00} & 1.00 & 3.75 & 5.81 & \textbf{4.00} & 4.34 & 3.86 & 4.18 & 4.49 & 4.42 & 3.74 & 5.04 & 5.03 \\ 
\hline
$\mathcal{M}_6$ & \textbf{6.00} & 36.00 & 8.50 & 8.00 & 12.00 & 9.00 & 12.00 & 1.00 & 11.95 & 12.00 & 1.00 & 6.00 & 8.43 & 2.00 & 7.34 & 6.25 & 6.91 & 7.16 & 7.12 & 5.87 & 8.76 & 8.52 \\ 
\hline
$\mathcal{M}_8$ & \textbf{12.00} & 19.00 & 10.00 & 15.50 & 24.00 & 17.00 & 24.00 & 2.00 & 23.77 & 24.00 & 1.00 & 11.33 & 17.95 & 5.00 & 14.43 & 10.00 & 14.24 & 13.21 & 13.83 & 13.80 & 11.99 & 19.50 \\ 
\hline
$\mathcal{M}_9$ & \textbf{20.00} & 16.00 & 9.00 & 14.50 & \textbf{20.00} & 11.00 & 19.00 & 1.00 & 19.86 & 9.00 & 1.00 & 13.48 & 19.07 & 3.00 & 15.12 & 10.00 & 15.14 & 13.49 & 15.25 & 14.77 & 19.00 & 19.41 \\ 
\hline
$\mathcal{M}_{10a}$ & \textbf{10.00} & 11.00 & 8.00 & 8.00 & 11.00 & 6.00 & 2.00 & 1.00 & 10.97 & 5.00 & 1.00 & 8.58 & 10.43 & 11.00 & 9.15 & 8.89 & 9.20 & 8.39 & 9.62 & 9.10 & 11.00 & 10.30 \\ 
\hline
$\mathcal{M}_{10b}$ & \textbf{17.00} & 14.00 & 13.00 & 13.00 & 18.00 & 10.00 & \textbf{17.00} & 1.00 & 17.88 & 8.00 & 1.00 & 12.80 & 17.10 & 4.00 & 13.96 & 10.00 & 13.90 & 12.47 & 14.20 & 13.96 & 18.00 & 17.29 \\ 
\hline
$\mathcal{M}_{10c}$ & \textbf{24.00} & 19.00 & 18.00 & 18.50 & 25.00 & 14.00 & 23.00 & 2.00 & 24.76 & 14.00 & 1.00 & 16.41 & 23.27 & 5.00 & 17.87 & 10.00 & 17.97 & 15.90 & 18.01 & 18.05 & 24.01 & 24.38 \\ 
\hline
$\mathcal{M}_{10d}$ & \textbf{70.00} & 54.00 & 49.00 & 50.00 & 71.00 & 39.00 & 69.00 & 3.00 & 69.05 & 35.00 & 1.00 & 31.62& \textbf{nan} & 71.00 & 36.65 & 10.00 & 37.17 & 31.47 & 34.71 & 39.85 & 71.00 & 69.95 \\ 
\hline
$\mathcal{M}_{12}$ & \textbf{20.00} & 15.00 & 8.50 & 15.00 & \textbf{20.00} & 11.00 & 11.00 & 1.00 & 19.82 & 11.00 & 1.00 & 12.74 & 20.30 & 6.00 & 16.04 & 10.00 & 16.22 & 13.98 & 15.47 & 17.04 & 12.05 & 19.79 \\ 
\hline
$\mathcal{M}n_1$ & \textbf{18.00} & 14.00 & 13.50 & 13.50 & 27.00 & 13.00 & 36.00 & 1.00 & 18.82 & \textbf{18.00} & 19.00 & 12.58 & 17.00 & 11.00 & 14.31 & 10.00 & 14.26 & 12.71 & 14.29 & 14.24 & 21.00 & 18.39 \\ 
\hline
$\mathcal{M}n_2$ & \textbf{24.00} & 20.00 & 17.00 & 17.00 & 36.00 & 18.00 & 48.00 & 1.00 & 25.08 & \textbf{24.00} & 25.00 & 15.42 & 23.30 & 16.00 & 17.87 & 10.00 & 17.85 & 15.63 & 17.49 & 18.26 & 31.00 & 24.85 \\ 
\hline
 $Mean_{error}$ &  &  0.65 &  0.29 &  0.26 &  0.33 &  0.39 &  0.54 &  0.88 &  0.28 &  0.45 &  0.67 &  0.21 &  0.14 &  0.46 &  0.18 &  0.32 &  0.17 &  0.23 &  0.17 &  0.16 &  0.15 &  0.11 \\ 
\hline

\end{tabular}
\end{adjustbox}
    \caption{Good datasets}
    \label{tab:my_label}
\end{table}

\begin{table}[]
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Method/Dataset & $\mathcal{M}_1$ & $\mathcal{M}_2$ & $\mathcal{M}_3$ & $\mathcal{M}_4$ & $\mathcal{M}_6$ & $\mathcal{M}_8$ & $\mathcal{M}_9$ & $\mathcal{M}_{10a}$ & $\mathcal{M}_{10b}$ & $\mathcal{M}_{10c}$ & $\mathcal{M}_{10d}$ & $\mathcal{M}_{12}$ & $\mathcal{M}n_1$ & $\mathcal{M}n_2$ & $Mean_{error}$ \\
\hline
ID & \textbf{10.00} & \textbf{3.00} & \textbf{4.00} & \textbf{4.00} & \textbf{6.00} & \textbf{12.00} & \textbf{20.00} & \textbf{10.00} & \textbf{17.00} & \textbf{24.00} & \textbf{70.00} & \textbf{20.00} & \textbf{18.00} & \textbf{24.00} & \\ 
\hline
PM & 9.00 & 2.00 & 2.00 & 8.00 & 36.00 & 19.00 & 16.00 & 11.00 & 14.00 & 19.00 & 54.00 & 15.00 & 14.00 & 20.00 & 0.65 \\ 
\hline
$PM_{Spec}$ & 8.00 & 2.00 & 3.00 & \textbf{4.00} & 8.50 & 10.00 & 9.00 & 8.00 & 13.00 & 18.00 & 49.00 & 8.50 & 13.50 & 17.00 & 0.29 \\ 
\hline
$PM_{Kmeans}$ & 8.00 & 3.50 & 5.00 & 5.50 & 8.00 & 15.50 & 14.50 & 8.00 & 13.00 & 18.50 & 50.00 & 15.00 & 13.50 & 17.00 & 0.26 \\ 
\hline
PFO & 11.00 & \textbf{3.00} & 5.00 & 8.00 & 12.00 & 24.00 & \textbf{20.00} & 11.00 & 18.00 & 25.00 & 71.00 & \textbf{20.00} & 27.00 & 36.00 & 0.33 \\ 
\hline
PFN & 7.00 & 2.00 & 2.00 & 5.00 & 9.00 & 17.00 & 11.00 & 6.00 & 10.00 & 14.00 & 39.00 & 11.00 & 13.00 & 18.00 & 0.39 \\ 
\hline
PMG & 1.00 & \textbf{3.00} & 2.00 & 1.00 & 12.00 & 24.00 & 19.00 & 2.00 & \textbf{17.00} & 23.00 & 69.00 & 11.00 & 36.00 & 48.00 & 0.54 \\ 
\hline
PRT & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 2.00 & 1.00 & 1.00 & 1.00 & 2.00 & 3.00 & 1.00 & 1.00 & 1.00 & 0.88 \\ 
\hline
PPR & 10.94 & 2.27 & 2.75 & 7.96 & 11.95 & 23.77 & 19.86 & 10.97 & 17.88 & 24.76 & 69.05 & 19.82 & 18.82 & 25.08 & 0.28 \\ 
\hline
PKS & 5.00 & 2.00 & 2.00 & \textbf{4.00} & 12.00 & 24.00 & 9.00 & 5.00 & 8.00 & 14.00 & 35.00 & 11.00 & \textbf{18.00} & \textbf{24.00} & 0.45 \\ 
\hline
PBS & 1.00 & \textbf{3.00} & 3.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 19.00 & 25.00 & 0.67 \\ 
\hline
CID & 8.91 & 2.87 & 3.58 & 3.75 & 6.00 & 11.33 & 13.48 & 8.58 & 12.80 & 16.41 & 31.62 & 12.74 & 12.58 & 15.42 & 0.21 \\ 
\hline
FSH & 11.02 & 2.92 & 3.34 & 5.81 & 8.43 & 17.95 & 19.07 & 10.43 & 17.10 & 23.27& \textbf{nan} & 20.30 & 17.00 & 23.30 & 0.14 \\ 
\hline
KNN & 11.00 & 4.00 & 1.00 & \textbf{4.00} & 2.00 & 5.00 & 3.00 & 11.00 & 4.00 & 5.00 & 71.00 & 6.00 & 11.00 & 16.00 & 0.46 \\ 
\hline
MADA & 9.62 & 3.07 & 4.14 & 4.34 & 7.34 & 14.43 & 15.12 & 9.15 & 13.96 & 17.87 & 36.65 & 16.04 & 14.31 & 17.87 & 0.18 \\ 
\hline
$Mind_{ML}$ & 9.10 & 2.90 & 3.77 & 3.86 & 6.25 & 10.00 & 10.00 & 8.89 & 10.00 & 10.00 & 10.00 & 10.00 & 10.00 & 10.00 & 0.32 \\ 
\hline
MLE & 9.53 & 3.03 & 4.03 & 4.18 & 6.91 & 14.24 & 15.14 & 9.20 & 13.90 & 17.97 & 37.17 & 16.22 & 14.26 & 17.85 & 0.17 \\ 
\hline
MOM & 8.60 & 2.79 & 3.77 & 4.49 & 7.16 & 13.21 & 13.49 & 8.39 & 12.47 & 15.90 & 31.47 & 13.98 & 12.71 & 15.63 & 0.23 \\ 
\hline
TLE & 10.10 & 3.13 & 4.21 & 4.42 & 7.12 & 13.83 & 15.25 & 9.62 & 14.20 & 18.01 & 34.71 & 15.47 & 14.29 & 17.49 & 0.17 \\ 
\hline
TNN & 9.28 & 2.92 & 3.79 & 3.74 & 5.87 & 13.80 & 14.77 & 9.10 & 13.96 & 18.05 & 39.85 & 17.04 & 14.24 & 18.26 & 0.16 \\ 
\hline
DANCo & 11.00 & 2.96 & 4.67 & 5.04 & 8.76 & 11.99 & 19.00 & 11.00 & 18.00 & 24.01 & 71.00 & 12.05 & 21.00 & 31.00 & 0.15 \\ 
\hline
ESS & 10.18 & 2.90 & 4.02 & 5.03 & 8.52 & 19.50 & 19.41 & 10.30 & 17.29 & 24.38 & 69.95 & 19.79 & 18.39 & 24.85 & 0.11 \\ 
\hline

\end{tabular}
\end{adjustbox}
    \caption{Good datasets}
    \label{tab:my_label}
\end{table}


\begin{table}[]
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Method/Dataset & $\mathcal{M}_{5a}$ & $\mathcal{M}_{5b}$ & $\mathcal{M}_7$ & $\mathcal{M}_{11}$ & $\mathcal{M}_{13a}$ & $\mathcal{M}_{13b}$ & $\mathcal{M}_{beta}$ & $\mathcal{M}p_1$ & $\mathcal{M}p_2$ & $\mathcal{M}p_3$ & $Mean_{error}$ \\
\hline
ID & \textbf{1.00} & \textbf{2.00} & \textbf{2.00} & \textbf{2.00} & \textbf{2.00} & \textbf{1.00} & \textbf{10.00} & \textbf{3.00} & \textbf{6.00} & \textbf{9.00} & \\ 
\hline
PM & 3.00 & 3.00 & 3.00 & 3.00 & 3.00 & 2.00 & 9.00 & 1.00 & 2.00 & 2.00 & 0.72 \\ 
\hline
$PM_{Spec}$ & 3.00 & 3.00 & 3.00 & 3.00 & 3.00 & 7.00 & 6.50 & 1.50 & 2.00 & 15.50 & 1.22 \\ 
\hline
$PM_{Kmeans}$ & 3.00 & 3.00 & 3.00 & 3.00 & 3.00 & \textbf{1.00} & 5.00 & 7.00 & 2.00 & 1.00 & 0.74 \\ 
\hline
PFO & 3.00 & 3.00 & 3.00 & 3.00 & 3.00 & 2.00 & \textbf{10.00} & 1.00 & 1.00 & 1.00 & 0.74 \\ 
\hline
PFN & 2.00 & \textbf{2.00} & \textbf{2.00} & 1.00 & 1.00 & \textbf{1.00} & 7.00 & 1.00 & 21.00 & 1.00 & 0.64 \\ 
\hline
PMG & 2.00 & \textbf{2.00} & 1.00 & \textbf{2.00} & 1.00 & 3.00 & 20.00 & 11.00 & 20.00 & 29.00 & 1.22 \\ 
\hline
PRT & \textbf{1.00} & 1.00 & 1.00 & 1.00 & 1.00 & \textbf{1.00} & 1.00 & 1.00 & 1.00 & 1.00 & 0.53 \\ 
\hline
PPR & 2.40 & 2.23 & 2.95 & 2.15 & 1.86 & 2.03 & 10.62 & 1.24 & 1.06 & 1.03 & 0.55 \\ 
\hline
PKS & 2.00 & \textbf{2.00} & 1.00 & \textbf{2.00} & 1.00 & 2.00 & \textbf{10.00} & 1.00 & 1.00 & 1.00 & 0.54 \\ 
\hline
PBS & \textbf{1.00} & 1.00 & 1.00 & 1.00 & \textbf{2.00} & 3.00 & 11.00 & 2.00 & 2.00 & 2.00 & 0.54 \\ 
\hline
CID & 1.01 & 2.79 & 1.96 & 1.97 & 1.94 & 4.01 & 3.47 & 2.14 & 2.63 & 2.92 & 0.57 \\ 
\hline
FSH & 2.91 & 2.91 & 2.88 & 1.97 & 2.88 & 1.97 & 5.27 & 0.90 & 0.89 & 0.89 & 0.72 \\ 
\hline
KNN & 3.00 & 1.00 & 3.00 & \textbf{2.00} & 1.00 & \textbf{1.00} & 40.00 & 1.00 & 21.00 & 30.00 & 1.20 \\ 
\hline
MADA & 1.08 & 3.17 & 2.09 & 2.10 & 2.08 & 3.78 & 6.64 & 3.07 & 5.14 & 6.55 & 0.44 \\ 
\hline
$Mind_{ML}$ & 1.00 & 2.37 & \textbf{2.00} & \textbf{2.00} & \textbf{2.00} & 1.20 & 6.31 & 2.90 & 5.08 & 6.52 & 0.12 \\ 
\hline
MLE & 1.06 & 2.82 & 2.07 & 2.07 & 2.06 & 1.75 & 6.63 & 3.04 & 5.19 & 6.64 & 0.21 \\ 
\hline
MOM & 1.17 & 2.86 & 2.01 & 2.21 & 1.93 & 1.83 & 5.78 & 2.73 & 4.22 & 4.76 & 0.28 \\ 
\hline
TLE & 1.11 & 2.91 & 2.14 & 2.16 & 2.13 & 1.84 & 6.21 & 3.13 & 5.34 & 6.70 & 0.24 \\ 
\hline
TNN & 0.98 & 1.97 & 1.94 & 2.02 & 1.96 & 1.00 & 6.54 & 2.99 & 5.48 & 7.23 & 0.07 \\ 
\hline
DANCo & \textbf{1.00} & 2.47 & 2.21 & 2.26 & 2.23 & \textbf{1.00} & 8.02 & 3.20 & 7.01 & 8.94 & 0.10 \\ 
\hline
ESS & 1.63 & 2.88 & 2.15 & 2.49 & 2.05 & 1.95 & 5.92 & 2.85 & 4.89 & 6.12 & 0.33 \\ 
\hline

\end{tabular}
\end{adjustbox}
    \caption{Bad datasets }
    \label{tab:my_label}
\end{table}
